SHIELD: LLM-Driven Schema Induction for Predictive Analytics in EV Battery Supply Chain Disruptions

The electric vehicle (EV) battery supply chain's vulnerability to disruptions necessitates advanced predictive analytics. We present SHIELD (Schema-based Hierarchical Induction for EV supply chain Disruption), a system integrating Large Language Models (LLMs) with domain expertise for EV battery supply chain risk assessment. SHIELD combines: (1) LLM-driven schema learning to construct a comprehensive knowledge library, (2) a disruption analysis system utilizing fine-tuned language models for event extraction, multi-dimensional similarity matching for schema matching, and Graph Convolutional Networks (GCNs) with logical constraints for prediction, and (3) an interactive interface for visualizing results and incorporating expert feedback to enhance decision-making. Evaluated on 12,070 paragraphs from 365 sources (2022-2023), SHIELD outperforms baseline GCNs and LLM+prompt methods (e.g., GPT-4o) in disruption prediction. These results demonstrate SHIELD's effectiveness in combining LLM capabilities with domain expertise for enhanced supply chain risk assessment.

==> Tables/news_dataset_info.tex <==
% Acquisition and Investment
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Acquisition and Investment} \\ \hline
Canada to invest \$2 billion on mineral strategy for EV battery supply chain \& China’s EV battery materials industry set for \$11bn capacity buildup \\ \hline
Why carmakers are pouring billions into new electric vehicle battery factories \& Private equity in talks with UK's BMI for EV battery exposure \\ \hline
CATL and Indonesia jointly build a nearly \$6 billion power battery industry chain project \& Durham battery storage company raises \$100 million \\ \hline
Volkswagen announces \$20 billion effort to build its own EV batteries \& Panasonic to open \$4B EV battery plant in Kansas \\ \hline
CATL announces construction of second European factory in Hungary \& Tesla co-founder’s startup gets \$2 billion to boost EV battery production \\ \hline
CATL and HGP establish partnership to jointly promote 5GWh battery energy storage application \& GM and POSCO Future M Investing \$1bn in North American EV Battery Supply Chain \\ \hline
Companies invest in EV battery factories in Europe \& Ecoprobm, sk on, ford investing in Québec; building cathode plant to solidify ev supply chain in north america \\ \hline
Redwood Materials raises \$1B to expand circular battery supply chain in US \& Nissan leads \$2.5 billion investment to build two more EVs in UK \\ \hline
\caption{Acquisition and Investment}
\end{longtable}

% Changes in Supply and Demand
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Changes in Supply and Demand} \\ \hline
How a battery shortage could threaten US national security \& EV battery report: Taiwan's rising role in the global supply chain \\ \hline
EV battery report: China remains dominant with growing production capacity and presence worldwide \& How a handful of metals could determine the future of the electric car industry \\ \hline
EV battery report: Malaysia may be dark horse in Southeast Asia's EV sphere \& Raw materials in short supply for EV makers struggling to meet customer demand \\ \hline
EV Has a Problem: 90\% of the Battery Supply Chain ‘Does Not Exist’ \& Do you like minting money?’: Musk urges entrepreneurs to enter lithium space as Tesla’s supply woes persist \\ \hline
Tin’s Critical Role in the Battery Supply Chain \& Surging EV sales hitting high lithium prices, supply chain constraints: experts \\ \hline
What is Vietnam’s Mining Capacity for EV Batteries? \& Supply Chain Disruptions in the Energy Industry: Challenges with the Supply of Lithium-ion Batteries \\ \hline
Making EVs without China’s supply chain is hard, but not impossible – 3 supply chain experts outline a strategy \& Ford's answer to EV supply chain hell: Cheaper batteries \\ \hline
Almost 400 new mines needed to meet future EV battery demand, data finds \& Power spike: How battery makers can respond to surging demand from Evs \\ \hline
China’s Battery Supply Chain Tops BNEF Ranking for Third Consecutive Time, with Canada a Close Second \& Canada vaults to second spot ahead of the U.S. in global EV battery-supply chain ranking \\ \hline
Is the EV Battery Supply Chain Ready for the Approaching Demand? \& Jump-starting electric car batteries: Will supply problems stall California’s mandate? \\ \hline
Chinese companies gain momentum in U.S. electric vehicle supply chain \& EV batteries: Can the West catch up with China? \\ \hline
China Has Perfectly Tangled The Battery Value Chain With Electric Vehicles - A Combo The U.S. And Europe Will Find Hard To Beat \& It's official: The battery crunch is the new chip shortage \\ \hline
An EV Talent Gap Will Weaken the U.S. Battery Supply \& Auto workers worry it takes less labor to build electric cars. Maybe not, some researchers say \\ \hline
Fear of cheap Chinese EVs spurs automaker dash for affordable cars \&  \\ \hline
\caption{Changes in Supply and Demand}
\end{longtable}

% Economic Environment
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Economic Environment} \\ \hline
Indonesia’s Battery Industrial Strategy \& DOE makes \$3.1B available for battery manufacturing incentives \\ \hline
Developing a resilient Canadian battery supply chain \& Battery Policies and Incentives Database Contributes to U.S. Efforts To Build a Secure Electric Vehicle Battery Supply Chain \\ \hline
US increases production to catch China in global battery race \& UK Inflation Rate Reaches 40-Year High As Food Prices Surge \\ \hline
The CHIPS Act Is Essential. So Is a Resilient EV Battery Supply Chain \& EV tax credits could stall out on lack of US battery supply \\ \hline
Electric Vehicle Battery Production May Lead To Coal Country’s Return \& Bank Of England To Get More Aggressive With 50 BPS Hike Later In The Week \\ \hline
Huge Tax Cuts Are Being Questioned By Investors As Pounds Sinks \& DOE taps 20 companies to receive \$2.8B for battery manufacturing, minerals processing build-out \\ \hline
The future of vehicles is electric': Biden announces \$2.8B for battery supply chain \& Canada Has an EV Edge, If It Acts Now \\ \hline
\$2.8B US EV supply-chain push appears to favor red states \& Biden Threatens Windfall Tax As He Accuses Oil Companies Of War Profiteering \\ \hline
Inflation Of The United Kingdom Jumps To 41-Year High Of 11.1\% \& Why Canada has the potential to become an EV battery supply chain powerhouse \\ \hline
US battery supply chain investments reach US\$92 billion since Biden took office \& China Sets 5\% As Their Economic Growth Target For 2023 \\ \hline
Ukraine Secures First IMF Loan To A Country At War \& Biden’s EV bet is a gamble on critical minerals \\ \hline
Largest Oil Refinery In Africa Launched By Aliko Dangote \& Dead EV batteries turn to gold with US incentives \\ \hline
DOE intends to award up to \$37M to advance EV battery recycling, transportation and design \& China’s Economy Experienced A Growth Of 6.3\% In The Second Quarter \\ \hline
China To Kickstart Economy, After Plans To Improve Internal Migration \& A 40\% Windfall Tax Was Approved By Italian Government As A Result Of Soaring Profits \\ \hline
France Plans To End The Use Of Fossil Fuels By 2030 \& South Africa Gets \$1 Billion Loan From World Bank To Tackle Power Crisis \\ \hline
\caption{Economic Environment}
\end{longtable}

% EV Enterprise Related
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{EV Enterprise Related} \\ \hline
VW and Bosch to upscale EV battery output in Europe \& Governor Ivey Joins Dura Automotive to Celebrate Grand Opening of High-Tech Factory in Muscle Shoals for EV Battery Enclosures \\ \hline
Auto Giants Race to Build U.S. EV Battery Assembly Plants \& CATL's German factory obtains battery cell production license \\ \hline
Automakers race to build EV battery supply chains in North America \& General Motors Fortifies EV Battery Supply-Chain Links \\ \hline
GM's North American battery supply chain is key to EV profits \& CATL's German factory successfully achieves battery cell production \\ \hline
The South is building the most vibrant EV and battery hub in the US \&  \\ \hline
\caption{EV Enterprise Related}
\end{longtable}

% Humanitarian and Ethical Crisis
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Humanitarian and Ethical Crisis} \\ \hline
Sudan protesters: Ready to die for freedom \& China’s electric vehicle battery supply chain shows signs of forced labor, report says \\ \hline
Amazon Rainforest Reaches Dire New Record For Deforestation \& Evacuees In Ukrainian Azovstal Iron And Steel Works Share Horror Stories \\ \hline
North Korea Announces its first Covid Outbreak Since The Start of The Pandemic: Triggers National Emergency \& One Month Since Burkina Faso’s Zinc Mine Trap: Miners’ Wives Pray For Miracles \\ \hline
Floods And Monsoon Rain Lead To Humanitarian Crisis In Pakistan \& Ukraine Government Confirm The Discovery Of 440 Bodies In Unmarked Graves \\ \hline
Gunman Attacks A Russian School In The City Of Izhevsk \& Coal Mine Plans To Crush UK Climate Goals \\ \hline
Chaos Erupt During The Arrest Of El Chapo’s Son, Leaves At Least 29 Dead \& Lethal Cough Syrup Kills 200 Children In Indonesia \\ \hline
EV battery imports face scrutiny under US law on Chinese forced labor \& Suicide Blast Kills At Least 54 People In Political Gathering In Pakistan \\ \hline
Aid Enters Into Gaza Through The Rafah Crossing Point \& Gaza Healthcare Collapses As Palestine Plunges Into Humanitarian Disaster \\ \hline
Foreign Nationals And Injured Palestinians Allowed Through Rafah Border Crossing \&  \\ \hline
\caption{Humanitarian and Ethical Crisis}
\end{longtable}

% Natural Disaster
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Natural Disaster} \\ \hline
Three Tiny Islands Have Borne the Brunt of Tonga’s Tsunami \& More than 30,000 displaced by floods in Indonesia’s Sumatra \\ \hline
Second Round Of Cyclone Hits Madagascar In The Space Of Two Weeks \& Heavy rains, landslides kill scores in Brazilian mountain city \\ \hline
Australian Flood Worsens As State Emergency Perform Evacuation \& Wildfire Spreads Near Chernobyl Disaster Site \\ \hline
Tornadoes Break Out In Texas As Weather Worsens And 23 Are Injured \& The Philippines Continue To Be Bombarded By Tropical Storm Megi \\ \hline
South Africa's Government To Begin Rebuilding After Disastrous Floods \& Floods From Heavy Rain Destroys Kabul Homes Killing 22 People \\ \hline
Thunderstorms In Quebec And Ontario With 5 Recorded Deaths \& Australia May Face A Summer Of Flood And Rains \\ \hline
Tens Of Thousands Of People Displaced Due To Flood In China \& Japan Faces Its Worst Recorded Heat Wave Since 1875 \\ \hline
Heatwaves And Wildfires Continue To Occur More Often \& Factories Were Forced To Close Down As China Experiences Worst Heatwave In 6 Decades \\ \hline
Half A Million People Affected By Flood In Nigeria, According To Emergency Reports \& More Than 80 People Reported Dead Trying To Escape Flood In Nigeria \\ \hline
Greenhouse Gases Reach Record High Levels In The Atmosphere \& Carbon Emission To Hit Record High In 2022 \\ \hline
Summer Heat Waves Estimated To Be Responsible For Up To 20,000 Deaths \& Scientists Reveal Rising Fetal Distress Due To Climate Change \\ \hline
60,000 People Reported With Covid-Related Death In China In Less Than 40 Days \& Eastern Asia Witnessing Extreme Cold Temperature \\ \hline
Turkiye And Syria Devastated By Massive Earthquake \& Wildfire Destroys Region In Russia With Extensive Damage To Infrastructure \\ \hline
Key Measures Predict That The Earth Is Falling Sick \& Pacific El-Nino To Increase The Heat Of The Planet In 2024 \\ \hline
Early Data Report Showing 2023 To Be Hottest Year On Record \& Heatwaves And Wildfire Smoke Sandwich The US In Fresh Climate Concerns \\ \hline
The World’s Hottest Day Recorded Since Recording Began In 1979 \& Panic In India As The Yamuna River Rises To Unprecedented Levels \\ \hline
Hail Storms Hit Italy, And A Fourth Heat Wave Predicted In Europe \& Flood Triggered In Hong Kong After A Heavy Typhoon \\ \hline
Australians Exposed To Smoke Blanket Following Hazard Reduction Burns \& New Reports Show That 10\% Of Swiss Glaciers Depleted In 2 Years \\ \hline
New Climate Discovery Shows September As The Hottest Month On Record \& Heavy Flood And Rain In Tanzania Kill 47 In Hanang District \\ \hline
Fumes And Fires After Volcanic Eruption In Iceland \&  \\ \hline
\caption{Natural Disaster}
\end{longtable}

% Political Issues
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Political Issues} \\ \hline
Nuclear Weapons Testing Resumed In North Korea, According To Surrounding Countries \& Amid Russian-Ukraine Crisis, Finland Pushes to Join NATO \\ \hline
Complete Reversal Of Trump’s Withdrawal As Biden Approves Redeployment Of US Troops To Somalia \& Turkey Moves To Block Finland And Sweden NATO Bid \\ \hline
Biden Pledges Support For Taiwan In A Statement That Has Raised Eyebrows \& Russian Diplomat Resigns In Geneva To Protest Against Russia-Ukraine Tensions \\ \hline
South Korea Says North Korea Launched 8 Short-Range Ballistic Missiles \& The US Has To Improve Bilateral Relationship, Says China’s Defense Chief \\ \hline
South Korea To Counter The North Korean Threat By Boosting Defense Capacity \& Tension In Taiwan Strait From China’s Military Activities \\ \hline
Third Aircraft Carrier Launched By China To Boost Military Might \& Islamic State Raids Medium Security Prison, Freeing Insurgents \\ \hline
Act As Partner, Not Opponent, China’s Wang Yi Tells Australia \& State Of Emergency Declared In Sri Lanka As The President Flees To The Maldives \\ \hline
Biden Assures The Middle East That United State Will Remain An Active Partner \& Ukraine President Zelenskiy Fires Spy Chief And Top State Prosecutor \\ \hline
Fresh Crisis Loom In Sri Lanka As Parliament Elects Ranil Wickremesinghe As President \& EU Has Launched Four Legal Cases Against the UK Over The Northern Ireland Protocol \\ \hline
Top Delegation From The US Visits Kyiv, Promises Their Continued Support \& Taiwan: Pelosi Departs Taipei Due To Sound Of Chinese Fury \\ \hline
An Arrest Warrant Has Been Issued In South Korea For The Developer Of The Cryptocurrency Luna \& The United States Has Been Accused By China Of Sending Dangerous Signals To Taiwan \\ \hline
In Anticipation Of United States Vice President’s Visit, North Korea Fire Ballistic Missile \& A Ballistic Missile Launched By North Korean Is Believed To Have Flown Over Japan \\ \hline
Coup Leader Ibrahim Traore Named As Transitional President Of Burkina Faso \& President Xi Jinping Announced That China Would Never Renounce The Right To Use Force Over Taiwan \\ \hline
Chief Of Cybersecurity In Germany Sacked Over Reports Of Ties With Russia \& A Rare Talk Between United States And Russia Defense Ministers, As They Discuss Ukraine War \\ \hline
Xi Jinping Begins His Third Term, Marking Him As The Most Powerful Leader Of China In Decades \& China Accused Of Establishing Illegal Police Station In The Netherlands \\ \hline
A Law To Mobilize Convicted Russians Has Been Signed By Putin \& European Union Calls For Urgent Joint Arm Purchase To Help Ukraine \\ \hline
Ballistic Missile Fired By North Korea Off East Coast \& Biden Visits Ukraine For The First Time Since Russia’s Invasion \\ \hline
China At G20 Meeting Calls For Joint Action In Debt Settlement \& President Of Honduras Confirms Her Country Has Switched Ties From Taiwan To China \\ \hline
International Criminal Court Issues Arrest Warrant For Russian President \& Immunity Granted To Putin And Bric Leaders By South Africa \\ \hline
Ceasefire Of 24 Hours In Sudan Announced By United States And Saudi Arabia \& Chinese Control Of Pirelli, Blocked By Italian Government \\ \hline
Former Security Officials In Ukraine Have Been Charged With Treason \& NATO Chief Confirms That Sweden’s NATO Bid Backed By Turkey \\ \hline
North Korea Launches Ballistic Missile After Threatening The United States \& President Of South Korea Promises Ukraine \$150m Aid \\ \hline
Zelenskiy Dismisses Ukraine’s Ambassador To London \& Niger’s President Removed, As Soldiers Announce Coup On National Television \\ \hline
Qatar Confirms the Extension of Ceasefire Between Israel And Hamas By Two Days \& President Putin Orders Increase In The Size Of Russian Military \\ \hline
President Putin Confirms He Would Run For Fifth Term As The President Of Russia \& General Assembly Of The United Nations Has Voted For An Immediate Ceasefire In Gaza \\ \hline
Russian Opposition Leader, Navalny Found In Remote Penal Colony \&  \\ \hline
\caption{Political Issues}
\end{longtable}

% Production Technology Progress
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Production Technology Progress} \\ \hline
The Transportation Transformation: Battery Research Today and Tomorrow \& CATL releases Kirin battery with global highest integration \\ \hline
Ford releases new battery capacity plan, raw materials details to scale EVs; on track to ramp to 600k run rate by ’23 and 2m+ by ’26, leveraging global relationships \& How the US plans to transform its lithium supply chain \\ \hline
Local, clean and circular supply chains: Panasonic advances EV battery tech \& How Lithium Batteries Can Power the US Economy \\ \hline
FORD TAPS MICHIGAN FOR NEW LFP BATTERY PLANT; NEW BATTERY CHEMISTRY OFFERS CUSTOMERS VALUE, DURABILITY, FAST CHARGING, CREATES 2,500 MORE NEW AMERICAN JOBS \& Electric Vehicle Battery Manufacturing Capacity in North America in 2030 is Projected to be Nearly 20 Times Greater than in 2021 \\ \hline
Ascend Elements Opens North America's Largest Electric Vehicle Battery Recycling Facility in Georgia \& Study unveils policy insights for reshoring EV battery production \\ \hline
Batteries: EVs to use silicon, solid state for next-generation batteries \& BMW powers Spartanburg with ‘local for local’ battery supply chain \\ \hline
New EV Battery Materials Will Beget New Dilemmas \& Panasonic needs four more EV battery plants, executive says \\ \hline
\caption{Production Technology Progress}
\end{longtable}

% Sign a Supply Agreement
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Sign a Supply Agreement} \\ \hline
LG Energy signs \$9bn EV supply chain deal in Indonesia \& GM signs agreement to source cobalt from Glencore \\ \hline
One-time tourist hotspot to supply key electric car battery ingredient for Stellantis \& CATL and FlexGen reach 10GWh battery energy storage system supply agreement \\ \hline
Stellantis signs non-binding supply deal for raw materials needed for EV batteries \& The U.S.-Zambia-DRC Agreement on EV Batteries Production: What Comes Next? \\ \hline
Honda signs supply deal with Ascend Elements for recycled battery materials \& Renault signs deal for EV battery supply with Verkor \\ \hline
Ford inks long-term lithium supply contracts \& Canada, Japan agree to work more closely on battery supply chains \\ \hline
Samsung SDI to supply EV batteries to Hyundai Motor starting 2026 \& Exclusive: US, Indonesia to discuss potential for deal on EV minerals \\ \hline
Honda, Mitsubishi Corp sign pact to optimise use of EV batteries \& CATL and Stellantis Group sign strategic memorandum of understanding to supply lithium iron phosphate batteries to Stellantis Group in European market \\ \hline
\caption{Sign a Supply Agreement}
\end{longtable}

% Trade Policy
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{Trade Policy} \\ \hline
As the US struggles to “green” supply chains, new EU battery regulation offers lessons \& UK Issues New Round of Targeted Sanctions Against Russia \\ \hline
Further Sanctions Against Russia Being Discussed By EU \& Gas Supplies To Poland And Bulgaria To Be Cut Off By Russia \\ \hline
Russian Billionaire Shields Assets From European Sanctions \& Singapore's National Dish Affected By The Malaysian Export Ban \\ \hline
Gulf States Sanction And Boycott India After Unwanted Remarks \& Russia’s Economy Will Be Hit By Further Sanctions \\ \hline
The New Climate Bill Demands All-American EV Batteries \& New US Climate Bill Seeks to Onshore Electric Vehicle Supply Chain \\ \hline
The Inflation Reduction Act places a big bet on alternative mineral supply chains \& China Sanctions Pelosi, Halts Cooperation With The United States Over Pelosi’s Taiwan Trip \\ \hline
China Vows To Take Countermeasures As The United States Approves \$1.1BN Arms Sales To Taiwan \& The New Climate Bill Demands All-American EV Batteries \\ \hline
Grain Export Deal Between Ukraine And Russia Brokered By United Nations Suspended By Russia \& U.S. Push to Secure EV Battery Supply Chains and the Role of China \\ \hline
U.S. strikes at China with EV battery deal \& EU Could End Reliance On Chinese Battery Supply Chain By 2030 Says T\&E \\ \hline
Ford-CATL Partnership Illustrates the Challenge of Decoupling EV Supply Chains \& Grain Deal Extended By Russia And Ukraine Amid Disagreement \\ \hline
G7 Request For Black Sea Grain Deal To Be Extended \& Russia Confirm It Will Not Renew Grain Deal With Ukraine \\ \hline
Ukraine Welcomes The Arrival Of First Grain Ships Using New Route \& Global EV battery supply chain puzzles over China graphite curbs \\ \hline
US-Canada Critical Mineral, EV Battery, and Semiconductor Cross-Border Supply Chain Issue \& New US rules on Chinese batteries could push up price of electric cars \\ \hline
China restricts exports of graphite as it escalates a global tech war \& China says Biden plan to shut it out of US battery supply chain violates WTO rules \\ \hline
US to limit Chinese firms, battery parts from winning EV tax credits \& Senator asks Treasury to bar Chinese battery firms, minerals from US EV tax credits \\ \hline
China Promise To Deepen Trade Ties With Vietnam \& Eight North Korean Sanctioned By South Korea Over Arms Trade \\ \hline
\caption{Trade Policy}
\end{longtable}

% War and Conflict
\begin{longtable}{|p{\textwidth}|}
\hline
\textbf{War and Conflict} \\ \hline
Russia’s War in Ukraine Reveals a Risk for the EV Future: Price Shocks in Precious Metals \& America Prepares for a Russian Invasion of Ukraine \\ \hline
Russia Launches Military Attack On Ukraine \& Russia-Ukraine conflict exposes risks in EV supply chains \\ \hline
Putin Progress In Donbas Slow But Visible Says Boris Johnson \& Ukraine Reports Extensive Damage To Nuclear Plants By Russian Rocket \\ \hline
A Recent Blast In Moscow Killed Daughter Of Putin Ally, Darya Dugina \& Zelensky Vows Ukraine Will Take Back Crimea When It Chooses \\ \hline
Prime Minister Of Ukraine Expresses Gratitude To Germany And Calls For More Weapons \& Zelensky Claims Significant Gains As Ukrainian Forces Retake A Key City \\ \hline
Russia Proclaims The Annexation Of Ukrainian Territory As Military Setback Looms \& Russia's Missile Strike Leaves Ukraine's Second City, Kharkiv, Without Power \\ \hline
Three People Dead After Drone Attack On Russian Bomber Base \& Russia Claims Victory After A Long Battle For The Salt Mine Town In Ukraine \\ \hline
Ukraine To Receive Leopard 2 Tanks From Germany \& Russian Strike Hits Center Of Ukraine, Kills Seven People \\ \hline
Russian Aircraft Destroyed By Ukrainian Drone \& Wagner Boss, Yevgeny Prigozhin, Listed As Part Of The Crew Of Plane Crash With No Survivors \\ \hline
Attack On Market In A Ukrainian City Has Killed At Least 17 People \& Several Missiles Has Been Launched By Ukraine On Crimea \\ \hline
Ukraine To Receive Long-Range Missiles From The United States \& Ukraine To Receive Seized Iranian Ammunitions From United States \\ \hline
Israel In Bid To Repel Militants Declares War Against Hamas \& Airstrike Hits Hospital In Gaza, Killing Over Hundred People \\ \hline
Missile Strike On Kharkiv Kills Six Postal Workers \& 15 People Confirmed Dead In An Israeli Attack On An Ambulance In Gaza City \\ \hline
Hospital In Gaza Has Been Surrounded By Israeli Tanks \& Israel-Hamas Truce Ends, As Israel Launches Attack On Gaza \\ \hline
\caption{War and Conflict}
\end{longtable}
